Classifying concepts via visual properties

We assume that substances in the world are represented by two types of concepts, namely substance concepts and classification concepts, the former instrumental to (visual) perception, the latter to (language based) classification. Based on this distinction, we introduce a general methodology for building lexico-semantic hierarchies of substance concepts, where nodes are annotated with the media, e.g.,videos or photos, from which substance concepts are extracted, and are associated with the corresponding classification concepts. The methodology is based on Ranganathan's original faceted approach, contextualized to the problem of classifying substance concepts. The key novelty is that the hierarchy is built exploiting the visual properties of substance concepts, while the linguistically defined properties of classification concepts are only used to describe substance concepts. The validity of the approach is exemplified by providing some highlights of an ongoing project whose goal is to build a large scale multimedia multilingual concept hierarchy.

==> S7_RelatedWork.tex <==
%As far as we know, this is the first time that a methodology is proposed where conceptual hierarchies are built from visual properties

%However, it allows us to refer to established works in the interface of vision and language resources. To that end, our work builds upon our own work in visual semantics \cite{giunchiglia2021a} and is in objective convergence with the huge amount of work done in exploiting lexical-semantics for visual recognition and image classification, for instance, see, e.g., . More specifically, our work in similar in spirit to that of ImageNet \cite{imagenet2009} but with several key differences. Firstly, the functional distinction between substance concepts and classification concepts which is pivotal for integrating vision and language. Secondly, we're founded on a conceptually sound \emph{logical framework} based on well-established and well-tested canonical principles which we use integrate to visual and lexical semantics. Thirdly, employing empirically established tenets in categorization, we elucidate what should be the nature of visual recognition at each level of a concept hierarchy. Finally, we're supported by the UKC \cite{fausto2017,giunchiglia2018} wherein we the language-agnostic concept core facilitates the integration of the recognition of visual concepts to over thousand languages.

%We also concentrate on the impact of formal ontologies on our work. Firstly, our work is broadly in sync with established work in ontology support and mediation for computer vision, see, among others \cite{maillot,ontocv}. The crucial distinction, again, lies in our work's integration of visual concepts and lexical concepts via a fine-grained mapping which is based \emph{tried-and-tested} canonical norms and categorization tenets, and additionally, in its novel utilization of the UKC as background knowledge. Secondly, with respect to formal ontological analysis, as has also been mentioned before, we logically ground the need for substance concepts and classification concepts on the ontological distinction, following \cite{guarino2002}, between perdurants and endurants respectively. Further, we note, from \cite{guarino2000}, that object similarity is a \emph{diachronic identity condition} as it facilitates re-identification of substances over time.  


